Transformer-Based Models for Question Answering on COVID19

In response to the Kaggle's COVID-19 Open Research Dataset (CORD-19) challenge, we have proposed three transformer-based question-answering systems using BERT, ALBERT, and T5 models. Since the CORD-19 dataset is unlabeled, we have evaluated the question-answering models' performance on two labeled questions answers datasets \textemdash CovidQA and CovidGQA. The BERT-based QA system achieved the highest F1 score (26.32), while the ALBERT-based QA system achieved the highest Exact Match (13.04). However, numerous challenges are associated with developing high-performance question-answering systems for the ongoing COVID-19 pandemic and future pandemics. At the end of this paper, we discuss these challenges and suggest potential solutions to address them.

==> cord-19-paper/name/ref.tex <==
@MISC{Lu,
author = {Zhuole Lu},
title = {[COVID] ALBERT Q&A→Ethical & Social Consideration
},
month = {April},
year = {2020},
howpublished={\url{https://www.kaggle.com/joljol/covid-albert-q-a-ethical-social-consideration}}
}
